On the Perturbed States for Transformed Input-robust Reinforcement Learning

Reinforcement Learning (RL) agents demonstrating proficiency in a training environment exhibit vulnerability to adversarial perturbations in input observations during deployment. This underscores the importance of building a robust agent before its real-world deployment. To alleviate the challenging point, prior works focus on developing robust training-based procedures, encompassing efforts to fortify the deep neural network component's robustness or subject the agent to adversarial training against potent attacks. In this work, we propose a novel method referred to as Transformed Input-robust RL (TIRL), which explores another avenue to mitigate the impact of adversaries by employing input transformation-based defenses. Specifically, we introduce two principles for applying transformation-based defenses in learning robust RL agents: (1) autoencoder-styled denoising to reconstruct the original state and (2) bounded transformations (bit-depth reduction and vector quantization (VQ)) to achieve close transformed inputs. The transformations are applied to the state before feeding it into the policy network. Extensive experiments on multiple MuJoCo environments demonstrate that input transformation-based defenses, i.e., VQ, defend against several adversaries in the state observations. The official code is available at https://github.com/tunglm2203/tirl

==> 6_bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/tungluu.jpg}}]{\textbf{Tung M. Luu}} (Graduate Student Member, IEEE) received B.Sc degree in electronic and telecommunication engineering from Hanoi University of Science and Technology, in 2017, and the M.Sc. degree in electrical engineering from Korea Advanced Institute of Science and Technology, in 2020. He is currently pursuing a Ph.D. degree with Korea Advanced Institute of Science and Technology. His research interests include machine learning, deep learning, and reinforcement learning.
\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/haeyong.jpg}}]{\textbf{Haeyong Kang}}(Member, IEEE), (S'05) received the M.S. degree in Systems and Information Engineering from University of Tsukuba in 2007. From April 2007 to October 2010, he worked as an associate research engineer at LG Electronics. With working experiences at the Korea Institute of Science and Technology (KIST) and the University of Tokyo, He received a Ph.D. at the School of Electrical Engineering, the Korea Advanced Institute of Science and Technology (KAIST) with a dissertation on forget-free continual learning in 2023. He is pursuing research such as unbiased machine learning and continual learning as a postdoctoral researcher at KAIST.
\end{IEEEbiography}

\vspace{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/HuuTri.jpg}}]{\textbf{Tri Ton}} (Graduate Student Member, IEEE). He received a B.Sc degree in Automation and Control Engineering from Ho Chi Minh University of Technology in 2021. He has been pursuing an M.Sc and Ph.D. degree at the Korea Advanced Institute of Science and Technology since 2022. His research interests are in computer vision, specifically focusing on 3D understanding.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/nguyen_xuan_thanh.jpg}}]{\textbf{Thanh Nguyen}} (Graduate Student Member, IEEE) received B.Sc degree in electronic and automation engineering from Ho Chi Minh City University of Science and Technology, in 2015. He has been pursuing an M.Sc. and Ph.D. degree in Korea Advanced Institute of Science and Technology since 2018. His research interests include machine learning, deep learning, and reinforcement learning.
\end{IEEEbiography}

\vspace{-1cm}
	
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/cdyoo.jpg}}]{\textbf{Chang D. Yoo}} (Senior Member, IEEE) He received the B.S. degree in Engineering and Applied Science from the California Institute of Technology, the M.S. degree in Electrical Engineering from Cornell University and the Ph.D. degree in Electrical Engineering from the Massachusetts Institute of Technology. From January 1997 to March 1999 he was Senior Researcher at Korea Telecom (KT). Since 1999, he has been on the faculty at the Korea Advanced Institute of Science and Technology (KAIST), where he is currently a Full Professor with tenure in the School of Electrical Engineering and an Adjunct Professor in the Department of Computer Science. He also served as Dean of the Office of Special Projects and Dean of the Office of International Relations, respectively.
\end{IEEEbiography}
